Safe Adaptation with Multiplicative Uncertainties Using Robust Safe Set Algorithm

Maintaining safety under adaptation has long been considered to be an important capability for autonomous systems. As these systems estimate and change the ego-model of the system dynamics, questions regarding how to develop safety guarantees for such systems continue to be of interest. We propose a novel robust safe control methodology that uses set-based safety constraints to make a robotic system with dynamical uncertainties safely adapt and operate in its environment. The method consists of designing a scalar energy function (safety index) for an adaptive system with parametric uncertainty and an optimization-based approach for control synthesis. Simulation studies on a two-link manipulator are conducted and the results demonstrate the effectiveness of our proposed method in terms of generating provably safe control for adaptive systems with parametric uncertainty.

==> sections/SEC2/20intro.tex <==
\color{black}In this section, we provide a mathematical description of dynamical systems with parametric uncertainty.\color{black}

==> sections/SEC3/30intro.tex <==
In this section, we provide a mathematical description of energy function based safe control problem.

==> sections/SEC4/42_SACL.tex <==
\color{red}From the formulation of the control problem in Section \ref{sec: roscp_SMSI}, it is apparent that the formulation does not account for parametric uncertainty. In order to extend the ideas of safe control to an adaptive system, we need to develop a new safety index that accounts for the unknown parameters yet does not change the underlying safety criterion. In other words, $\mathcal{X}_s$ must remain the same. Thus to highlight this fact, we explicitly state that dependence with a new safety index we denote as $\phi_{AC}(x,\hat{\xi}): \mathcal{X} \times \mathcal{P} \rightarrow \mathbb{R}$. This safety index is dependent on the estimate of the true parameter because the true parameter is not available to evaluate the expression. If $\phi_{AC}$ is designed to satisfy the conditions in Def.~\ref{def: sufficient}, then the underlying safety criterion is not changed and the adaptive system is safe under an adaptive control law that satisfies the following condition:
\begin{equation}\label{eq: phi dot ac}
    \dot{\phi}_{AC}(x, \hat{\xi}) \leq -\eta,  \forall \text{ } (x,\hat{\xi}) \in \{ (x,\hat{\xi}): \text{ } \phi_{AC}(x,\hat{\xi}) \geq 0\}.
\end{equation}
Equation \eqref{eq: phi dot ac} is a straight one-to-one translation from \eqref{eq: phi dot}. Nonetheless, it is important to notice that the time derivative of the safety index also depends on the adaptation law:
\begin{subequations} \label{eqESI3}
\begin{align}
        \dot{\phi}_{AC}(x, \hat{\xi}) &= \nabla_{x}\phi_{AC}^T(x,\hat{\xi})\dot{x} +\nabla_{\hat{\xi}}\phi_{AC}^T(x,\hat{\xi})\dot{\hat{\xi}}, \\
           &= \begin{aligned}[t]\nabla_{x}\phi_{AC}^T(x,\hat{\xi})(f(x, \xi) + g(x, \xi)u) \\
           +\nabla_{\hat{\xi}}\phi_{AC}^T(x,\hat{\xi})\dot{\hat{\xi}},
        \end{aligned}\\
        &= L_f\phi_{AC} + L_{g}\phi_{AC}u + \nabla_{\hat{\xi}}\phi_{AC}^T(x,\hat{\xi})\dot{\hat{\xi}},
\end{align}
\end{subequations}

where $L_f\phi_{AC}:=\nabla_{x}\phi_{AC}^T(x,\hat{\xi})f(x, \xi)$ and $L_{g}\phi_{AC}:=\nabla_{x}\phi_{AC}^T(x,\hat{\xi})g(x, \xi)$ are Lie derivatives.  
This distinction is important as we see from the expansion of the safety index (inspired by \cite{TC_SCAUEF}).

In order to leverage the performance advantages of an adaptive controller, as well as the safety guarantees arising from the use of an energy function based safety controller, we propose a safe adaptive control algorithm based on the ideas of the Safe Set Algorithm. In this algorithm, the auxiliary safety controller only influences the system when the system is about to violate the safety criterion. In particular, the proposed method is motivated by the approach in \cite{LT_CIASS}, which leverages an optimization framework for safe control. This basic form of the controller follows from a general auxiliary safe controller, \textit{i.e.}:
\begin{equation}
     u_{\text{safe}} =
    \begin{cases}
      k(x, \hat{\xi}) - cL_{g}\phi_{AC}^{T} & \text{ if $\phi(x,\hat{\xi}) \geq 0$}\\
      k(x, \hat{\xi}) & \text{otherwise.}
    \end{cases}
\end{equation}

However, as this formulation revolves around being able to calculate the true direction of the Lie derivative of the control, which is dependent on a set of unknown parameters, we must modify this approach to utilize the estimate of that direction:
\begin{equation} \label{control}
     u_{\text{safe}} =
    \begin{cases}
      k(x, \hat{\xi}) - c\widehat{L_{g^*}\phi_{AC}^{T}} & \text{ if $\phi(x,\hat{\xi}) \geq 0$}\\
      k(x, \hat{\xi}) & \text{otherwise,}
    \end{cases}
\end{equation}
where the constant $c$ is selected such that \eqref{eq: phi dot ac} is satisfied. The term, $k(x, \hat{\xi})$, serves as the controller when the safety constraints are not at risk of being violated, and in this work is assumed to be an adaptive controller whose stability properties are verified independently of the safety controller. \color{black}
